Handbook of derivative AdS amplitudes

In the 2022 study, together with Paul McFadden and Kostas Skenderis, I analyzed tree-level 3- and 4-point Witten diagrams (amplitudes) of scalar operators in anti-de Sitter space in momentum space. This paper constitutes its extension to Witten diagrams with bulk interactions involving spacetime derivatives. In $d = 3$ boundary dimensions the Witten diagrams involving conformally coupled and massless scalars can be evaluated in closed form. Such cases are of interest in holographic cosmology and correspond to dual operators of conformal dimensions $\Delta = 2$ and $3$ respectively. I present explicit formulae for all such amplitudes and provide a Mathematica package serving as the repository of all the results. I discuss renormalization issues and show that, contrary to the expectation, even finite correlators may acquire non-trivial renormalization effects.

==> package/HypExp/HPLInstall <==
#!/bin/bash
Minimalsetlist=`ls MinimalSet?.m`
Minimalsetlistpm=`ls MinimalSetpm?.m`
htablelist=`ls h?table.mat` 
HPLatIlist=`ls HPLatI?.m` 
numHPLatIlist=`ls numHPLatI?.m` 

HPLExecutables="HPLUninstall"
filestocopy="$htablelist $Minimalsetlist $HPLatIlist $numHPLatIlist $Minimalsetlistpm  nmzv.m .HPLversion "


possibleinstallationpath="$HOME/HPL $PWD Other"


function hpl_find_platform() {


case $HOSTTYPE in 
*linux* ) platform=linux ;;
power_pc|intel_pc|*mac*|powerpc) platform=mac ;;
*) echo "Could not determine the type of platform, please choose the most appropriate:";
platforms="mac linux";
select platform in ${platforms};
do
    if  [ -z $platform ] ; then
    	echo "Please choose a number between 1 and 2"
    fi
    break
done
;;
esac
case $platform in 
linux) initmdir=$HOME/.Mathematica/Autoload ;;
mac) initmdir=$HOME/Library/Mathematica/Autoload ;;
esac
echo "Platform: "$platform
}

function find_old_version() {

OldHPLPath=`grep "HPLPath =" $initm | grep -o "\".*\""| grep -o "[^\"].*[^\"]"`
#OldHPLPath=`sed -n "/HPLPath =/{s/\\\$HPLPath = \"\(.*\)\"/\1/;p}" $initm`
#thisHPLversion=`sed -n "/HPL/s/HPL version \([0-9].[0-9]\)/\1/;p" .HPLversion`
thisHPLversion=`grep -o "[0-9].[0.9].*"  .HPLversion`
if [ -e $OldHPLPath/.HPLversion ] ; then
#thatHPLversion=`sed -n "/HPL/s/HPL version \([0-9].[0-9]\)/\1/;p" $OldHPLPath/.HPLversion`
thatHPLversion=`grep -o "[0-9].[0.9].*" $OldHPLPath/.HPLversion`
else thatHPLversion="0.0"
fi

if [ "$thatHPLversion" == "$thisHPLversion" ]; then
    echo "Version  $thatHPLversion is already installed in 
    	$OldHPLPath, 
do you want to reinstall it somewhere else or overwrite it ?"
    choices="reinstall overwrite abort"
    select choice in ${choices};
    do 
    case $choice in
    	reinstall)  use_old_path="false";    break ;;
    	overwrite) use_old_path="true"; HPLPath=$OldHPLPath;   break ;;
    	abort) exit 0 ;;
    	*) echo "Please enter either 1,2 or 3"
    esac
    done

else 
echo "There is already a version of HPL installed (version $thatHPLversion), the version this script installs is $thisHPLversion. 
Do you want to replace 
     version $thatHPLversion 
with 
     version $thisHPLversion?"
choices="replace abort"
select choice in ${choices};
do 
case $choice in
    replace)     break ;;
    abort) exit 0 ;;
    *) echo "Please enter either 1 or 2"
esac
done
fi
}




function copy_files() {
if [ $HPLPath != $PWD ] ; then 
    [ -e $HPLPath/HPL.m ] && {
    	echo "There is already a version of HPL.m in the directory..."
    	echo -n "Deleting old version........................"
    	rm $HPLPath/HPL.m
    	echo  "Done"
    	}
    echo -n "Copying the package HPL.................."
    cp -f $PWD/HPL.m $HPLPath
    echo  "Done"

    echo -n "Copying the auxiliary files................."
    
    chmod +x $HPLExecutables
    cp -f $HPLExecutables $HPLPath
    
    cp -f  $filestocopy $HPLPath
    
    echo  "Done"
fi

}

function choose_install_dir() {
echo "Please select the name of the directory where"
echo "the package should be installed."
echo 
select installationpath in ${possibleinstallationpath};
do
    if ! [ -z $installationpath ] ; then
        if [ $installationpath == Other ]; then
        	echo "Please give the full path of the directory to install the package:"
        	read useripath
        	echo
		mkdir -p $useripath || { echo "unable to create directory, exiting...";exit; }
	   	ipath=$useripath   		
    	else
    	    ipath=$installationpath;
    	fi
    	break;
    else 
    	echo "Please choose a number between 1 and 3}"
    fi
done
echo
echo "installing package in $ipath ..."

HPLPath=$ipath

if ! [ -d $HPLPath ]; then
    mkdir -p $HPLPath ;
fi

}

# install_init_m 

function install_init_m() {
echo "(* begin of the lines added by HPL *)">install.m
echo "\$HPLPath = \"$HPLPath\"" >> install.m
echo "If[Not[MemberQ[\$Path,\$HPLPath]],\$Path = Flatten[{\$Path, \$HPLPath }]];">>install.m
echo "(* end of the lines added by HPL *)">>install.m

grep "HPLPath" $initm >& /dev/null && { 
    echo "Found HPL lines in initialisation file, replacing with new........."
    sed "/begin of the lines added by HPL/,/end of the lines added by HPL/d" $initm >HPL.init.m.temp
    cp HPL.init.m.temp $initm; rm HPL.init.m.temp;echo "Done" 
}  
cat install.m >> $initm;
}

function find_math {

MATH=""
echo "Locating mathematica executable ..."
which MathKernel >& /dev/null && { 
    MATH=`which MathKernel`
    } || { 
    which math >& /dev/null && { 
    	MATH=`which math`
    }
}

if [ -z $MATH ] ; then 
    echo "not found, trying harder... " 
    all=`locate MathKernel | grep '/MathKernel$'`
    allex=""
    for file in $all ; do
    	if [ -x $file ] ; then 
    	    allex="$allex $file"; 
    	fi
    done
    echo
    echo "The following executables have been found, please choose the one that should be used to check the installation. If you don't want to check the installation, choose \"none\", if you want to provide another executable, choose \"other\" 
"
    choices="$allex other none"
    while [ -z $MATH ] ; do
    	select choice in ${choices};
    	do 
    	    case $choice in
    	    	none) MATH="none";return 1 ; break ;;
    	    	other) read MATH ;break ;;
    	    	*) MATH=$choice; break ;;
    	    esac
    	done
    	if ! [[ -x $MATH ]] ; then
    	    echo "The executable could not be found, please try again."
    	    MATH=""
    	fi
    done
fi
echo "using 
$MATH 
as path for the mathematica executable."
}


function check_install(){
    MATH=""
    find_math && {
    	$MATH -run "Quit[]" < HPLnolicense >& /dev/null ||{
    	    failure=math
	    return 1
    	}	
        $MATH < HPLInstallTest.m >& /dev/null && {
    	    echo "Installation successful!"
    	    echo 
    	    echo The package can now be called with:
    	    echo
    	    echo  "    \" <<HPL\` \" "
    	    echo
    	    return 0
        }
    	failure=initm
    	return 1
    }
    failure=math
    return 1
}

function kernel_trick() {
    Kinitm=$initmdir/../Kernel/init.m
    echo "Get[ToFileName[\"$initmdir\",\"init.m\"]]" >> $Kinitm; 
}

echo
echo 
echo "*********************************************"
echo This installs the HPL Mathematica Package...
echo "*********************************************"
echo

hpl_find_platform
initm=$initmdir/init.m


grep "HPLPath" $initm  >& /dev/null && { find_old_version; }
if ! [ "$use_old_path" == "true" ] ; then choose_install_dir; fi
copy_files    
echo -n "Checking installation: .... "
install_init_m

check_install || {
    case $failure in 
    	math) echo "The installation could not be checked since the command math could not be run." ; return 0 ;;
    	initm)	kernel_trick;; 
    esac
    check_install || {
    	echo Installation check failed 
    } 
}    



==> package/HypExp/HPL_README <==
%%%%%%%%%% HPL %%%%%%%%%%%%%% 

The Mathematica package HPL  is an implementation of the harmonic polylogarithms (HPL) of Remiddi and Vermaseren. The package contains implementation of

-the product algebra,
-derivatives,
-some simple integrations
-reduction to more common functions (log's, polylog's, Nielsen polylog's)
-singular behaviour extraction
-analytic continuation (with control over the sign of the imaginary parts)
-change of arguments (x = -t,x = t²,  x = 1-t, x =  1/t , x =  t/(t-1), x = (1-t)/(1+t)  )
-numerical evaluation
-values at argument 1, multiple zeta values (MZV's)

A detailed description and many examples can be found in  hep-ph/0507152

------------------------------------
Installation (Linux)
------------------------------------

There is an installation program with the package. It copies the files where they belong, updates your init.m file, so that you can load the package without having to give the whole path.

To install the package, copy the tar file HPL-N.x.tar.gz  to your disk, unpack it with

> gunzip HPL-N.x.tar.gz
> tar -xf  HPL-N.x.tar

Change directory to the HPL-N.x directory

> cd  HPL-N.x

Change the permission of the installation script:

> chmod +x HPLInstall

Execute it:

> ./HPLinstall

Follow the instruction...

------------------------------------
Installation (Windows)
------------------------------------

There is no installation script for Windows. It copies the files where they belong, updates your init.m file, so that you can load the package without having to give the whole path.

To install the package,

- copy the tar file HPL-N.x.tar.gz  to your disk, where you want the package to be,

-unpack it

-copy and download in the directory HPL-N.x all the additional tables (see below) you need (this can also be done afterwards).

The package can be called with

$HPLPath="the:\path\of\the\installation"

Get[ToFileName[{$HPLPath},"HPL.m"]]

If you do not want to type this each time, you can add the following lines to your init.m file in the AutoLoad directory of your Mathematica installation.

$HPLPath="the:\path\of\the\installation"
$Path=Flatten[{$Path,$HPLPath}]

In the next sessions you can then load the package with <<HPL` only.

------------------------------------
Additional tables for weights higer than 6
------------------------------------

The reduction to a minimal set and the values at one and i requires quite large tables. In order not to use unnecessarily the memory, the tables for weight higer than 6 are not included in the basis package (the HPL-N.x.tar.gz file). If the user needs the HPL's of weight higher than 6, he can simply add the required files into the installation directiory of HPL and unzip them (> gunzip MinimalSet?.m.gz). The new tables will be loaded automatically in the next Mathematica session.

The additional tables can be downloaded from the home page:

http://krone.physik.unizh.ch/~maitreda/HPL/

------------------------------------
Uninstall HPL
------------------------------------

Under Linux, run the program

> ./HPLuninstall

in the installation directory of  HPL. Under Windows remove the files of the installation.

------------------------------------
Bug reports
------------------------------------

Great care has been taking in testing  the HPL package.  However, if there were problem left we would appreciate to get bug reports. Please use the Email  address of the home page 

http://krone.physik.unizh.ch/~maitreda/HPL/

to send bug reports. 

--- last update: 14 sept 2005



==> package/HypExp/README <==
The package HypExp

The Mathematica package HypExp allows to expand arbirtary hypergeometric functions JFJ-1 around their parameters. A detailed description can be found in  hep-ph/0507094

-------------------------------------------------------------
 Installation under Linux 
-------------------------------------------------------------

There is an installation program with the Package. It copies the files where they belong, updates the init.m file in the .Mathematica/Autoload/ directory in the home directory, so that you can load the package without having to give the whole path.  It also installs the package HPL which is used by the package HypExp.

To install the package, copy the tar file HypExp-1.0.tar.gz  to your disk, unpack it with

> gunzip HypExp-1.1.tar.gz
> tar -xf  HypExp-1.1.tar

Change directory to the HypExp-1.1 directory

> cd  HypExp-1.1

Copy in this directory the lib*.tar.gz file from the homepage 

    http://krone.physik.unizh.ch/~maitreda/HypExp/

corresponding to the libraries you want to install (it is possible to install other libraries afterwards, see below).

Change the permission of the installation script:

> chmod +x HypExpInstall

Execute it:

> ./HypExpInstall

Follow the instruction...

-----------------------------------------------------------------
HypExp installation for Windows
-----------------------------------------------------------------

There is no script which automatically installs HypExp under Windows. If you want to use HypExp under Windows you should follow the following steps:

- Download the file HypExp-win-1.1.tar.gz

- Unpack it in the directory where you want HypExp to be installed

- In this directory you find a file called init.m, modifiy the first line such that your installation path replaces

              the:\path\of\the\installation

- To load the package you have to type in Mathematica

Get[ToFileName[{"the:\path\of\the\installation"},"init.m" ]]

<<HypExp`

If you don't want to type the first line each time, you can add the content of the init.m file of HypExp to the init.m file in the AutoLoad directory of your Mathematica installation. You will then only need to type the second line.

------------------------------------------------------------------
Libraries
------------------------------------------------------------------

The libraries avoid recalculating the same expansions each time they are needed. It makes the use of the package much more efficient.

They can be found on the webpage of HypExp: 

http://krone.physik.unizh.ch/~maitreda/HypExp/

The HypExp libraries can be read from Maple, more info on this can be found at 

http://krone.physik.unizh.ch/~maitreda/HypExp/Maple.html

------------------------------------------------------------------
Installing new libraries under Linux
------------------------------------------------------------------

To install new libraries, copy the corresponding lib*.tar.gz file(s) to the installation directory of the Package (if you do not remember, the Mathematica variable $HypExpPath contains it...).  Run then the programs install_libs and lib_consistency (and NOT make_lib...)

> ./install_libs
>./lib_consistency

That's it.

------------------------------------------------------------------
Installation of the libraries for Windows
------------------------------------------------------------------

Here again, the procedure is not automated for Windows, you should follow these steps:

- copy all the library files (lib*.tar.gz and the corresponding install_lib*.m) you want in your installation directory. These libraries can be found on the HypExp Homepage.

- unpack them

- copy  the install_lib*.m file for each library in the installation directory.

- run for each install_libXXX.m file

>cd  the:\path\of\the\installation
> math< install_libXXX.m

in the command line.

------------------------------------------------------------------
Uninstall HypExp
------------------------------------------------------------------

Run the program

> ./HypExpUninstall

in the installation directory of HypExp.

------------------------------------------------------------------
Bug reports, bug fixes, new versions
------------------------------------------------------------------

Great care has been taken in testing  the HypExp package.  However, if there are problems left we would appreciate to get bug reports to the adress found on the HypExp homepage. If you want to get informed upon bug fixes and new versions, please send us your address.

-------------------------------------------------------------------
More Infos
-------------------------------------------------------------------

http://krone.physik.unizh.ch/~maitreda/HypExp/

